FreshDiskANN: A Fast and Accurate Graph-Based ANN Index for Streaming Similarity Search

Approximate nearest neighbor search (ANNS) is a fundamental building block in information retrieval with graph-based indices being the current state-of-the-art and widely used in the industry. Recent advances in graph-based indices have made it possible to index and search billion-point datasets with high recall and millisecond-level latency on a single commodity machine with an SSD. However, existing graph algorithms for ANNS support only static indices that cannot reflect real-time changes to the corpus required by many key real-world scenarios (e.g. index of sentences in documents, email, or a news index). To overcome this drawback, the current industry practice for manifesting updates into such indices is to periodically re-build these indices, which can be prohibitively expensive. In this paper, we present the first graph-based ANNS index that reflects corpus updates into the index in real-time without compromising on search performance. Using update rules for this index, we design FreshDiskANN, a system that can index over a billion points on a workstation with an SSD and limited memory, and support thousands of concurrent real-time inserts, deletes and searches per second each, while retaining $>95\%$ 5-recall@5. This represents a 5-10x reduction in the cost of maintaining freshness in indices when compared to existing methods.

==> 1b-run.tex <==

%% \noindent\textbf{\algofresh}. Our experiments described 
%% in ~\Cref{subsec:algofresh_recall_stability} are run on the \texttt{mem}
%% machine with 64-threads for batch insert and delete operations. 
%% We present effective latencies for both insert and delete operations 
%% in ~\Cref{fig:ramp-up-100M}. Delete operations can be easily
%% handled by writing to a \emph{stop} list temporarily. However,
%% accumulating a large number of deletes in the stop list can degrade
%% search performance. Only for the purpose of this experiment, we
%% incorporate the time taken to reflect those changes in the \algofresh
%% index into the delete latency. As expected, with increasing index
%% size, both insert and delete operations take longer, but consistently
%% stay under 10ms per operation end-to-end.

\input{plots/latency-ramp-up-1b}

\subsection{Practical \diskanntwo deployments}\label{subsec:ssd-perf}
We now simulate realistic use-cases for \algofresh and \diskanntwo through experiments with ramp-up and steady-state indices. 

\noindent\textbf{Ramp-up Index}.We start with a \diskanntwo index built on 100M points randomly sampled
from SIFT1B, and grow the index over time through disproportionately higher
insertions as compared to deletions. We use $R=64, L_c = 75,$ and
$\alpha=1.2$ for all experiments with \algo, \algofresh, \diskann, and
\diskanntwo for comparison of performance and quality.

In each cycle, in the foreground, 3 threads randomly sample 
30M points from the spare pool and insert them into the index, while 10 threads
execute search on the entire \diskanntwo index using a query set with 10,000 queries repeatedly. 
Once 30M points are inserted into the \textbf{RW-\tempindex} index, a background thread coverts it into a
\textbf{RO-\tempindex}, a new \textbf{RW-\tempindex} instance is brought up with 0 points, and the \texttt{\merger} procedure(\Cref{sec:final-design}) is triggered with 80, 40, and 80 threads for the
\texttt{DELETE}, \texttt{INSERT}, and \texttt{PATCH} phases
respectively. The foreground threads continue their insert
and search operations while merge progresses in the background. 
This results in resource contention for SSD access which reduces 
throughput for both operations. Once the background merge is complete,
we atomically swap the current \lti index with the output merged
\lti index. This also removes any \textbf{RO-\tempindex} instances whose changes were merged into the new \lti. 
We run this experiment till the \diskanntwo size reaches
800M points. This takes about 3 days to execute on the \texttt{ssd}
machine with a maximum memory footprint consistently under $128$GB.

\Cref{fig:ramp-up-1b-search-latency,fig:ramp-up-1b-insertion-latency}
show the \emph{user-perceived} search latency and insert throughput
respectively throughout the ramp up. We adjust search parameters to
consistently provide $\recall{5}{5} > 90\%$ on the entire \diskanntwo index
at all times. We notice that the query latency, while no
more than tens of milliseconds, fluctuates in phases. Although the \texttt{\merger}
procedure executes in the background, during its \texttt{Insert} phase, it generates a significant number of random reads to a \emph{consolidated} index that interfere with
the random read requests issued by the foreground search threads resulting in higher
latencies (and worse throughput) for both types of reads. Further, during the \texttt{Delete} and \texttt{Patch} phases of \texttt{\merger}, query search latencies spike as high as 40ms, presumably due to head-of-line blocking by the large sequential read and write operations that stream the \lti index to and from the main memory. 

%?? TODO ??
%To combat this latency spike, we reduce the granularity of our sequential I/O for the \texttt{Delete} and \texttt{Patch} phases from 256MB to 4MB per I/O operation. 
%In addition, we pipeline read and write operations with the compute to further reduce effective bandwidth consumed by our background operations. 
%We present a head-to-head comparison of the distribution of the 99th percentile query search latency over a 24-hour duration of identical steady-state experiments \Cref{fig:steady-800m-search-latency-99th}. 
%As expected, reducing the granularity of our sequential I/O reduces the effects of head-of-line blocking on the tail latency for query search. 
%We observe in the second plot that there are no latency spikes over 200 ms while in the the first plot these spikes go as high as 250ms.
%To further illustrate this comparison \Cref{fig:steady-800m-search-latency-99th-hist} shows a frequency distribution of these search latencies in the two experiments.


%% Since merge procedure uses Product-Quantized
%% representations for distance comparisons during both \texttt{DELETE}
%% and \texttt{PATCH} phase, we expect the quality of the output \diskann
%% indices to worsen over time, increasing the query latency. From
%% \Cref{fig:fig9}, we see that query latency increases as the graph
%% quality decreases over time, before saturating. This trend is similar
%% to the stabilization of recall as shown in \Cref{fig:ramp-up-1b}.

 \noindent\textbf{Steady-state Index}. We initialize this experiment with 
 the output of the above ramp-up experiment -- a \diskanntwo index
 containing $\approx$800M points. To simulate a \emph{steady-state} 
 deployment of \diskanntwo, we request all three operations --
 insert, delete, and search -- in the foreground while the merge
 procedure executes in the background. We run this experiment for multiple cycles,
 in each of which 30M randomly chosen points from the \diskanntwo
 index are deleted and another set of 30M points are inserted from the spare pool of 200M points.
 We allocate 40 threads for all phases of the background \texttt{\merger} procedure, and 2, 1,
 and 10 threads each for insert, delete, and search operations
 respectively. We run this experiment for 10 cycles amounting to 
 about 2 days of runtime on the \texttt{ssd} machine with a maximum memory
 footprint of under 128GB. We present \emph{user-perceived} latencies
 for search and insert operations on \diskanntwo in
 ~\Cref{fig:steady-800m-search-latency,fig:steady-800m-insert-latency}.
 
\noindent\textbf{Throttling update operations}. While \diskanntwo
provides latencies of about $1$ms for insert operations and about
$0.1\mu$s for delete operations, in practice, both operations need to
be throttled so the in-memory \tempindex does not grow too large
before the background merge concludes and is ready to push the new changes to the new \lti. 
In effect, the speed of the merge operations dictates the update rates the system can sustain over long
periods of time. Accordingly, for both experiments in this
subsection, we under-allocate threads for update operations and
allow the \texttt{\merger} procedure to consume more than half the threads in system to limit the
size of \tempindex below $\leq 30$M while merge completes.

In the ramp-up experiment where the index grows without any delete operations, the
merge takes a maximum of $8400$s to insert $30$M points into the \lti. We conclude
that the system can support around $\frac{30,000,000}{8400}\approx3570$ inserts/second without
backlogging the merge, when no delete requests are issued.

In the steady-state experiment where the index maintains a constant size of about
800M points is updated in cycles of equal sized insertions and deletions of 30 million points, the
\texttt{Delete} phase takes a maximum of 10280 seconds, and the overall
\texttt{\merger} procedure takes about 16277 seconds. Following a similar of reasoning as before, 
we conclude that the system can support at least 1840 inserts \textbf{and} deletes per second without
backlogging merge, for a total of $\approx 3680$ update operations per second.

\noindent\textbf{Merge and Search throughput}. We vary the number of merge threads from 10 to 40 and record the merge time for merging 30M inserts and deletes into a 800M index in \Cref{tab:merge-time-800M}. 
In \Cref{fig:800m-search-latency}, we show the trend of mean and 99th percentile search latencies with increasing number of threads for search on 800M index. 
Lastly, in \Cref{fig:800m-search-throughput}, we show the trend of search throughput for the same.

\begin{table}
  \centering
  \caption{Merge time with different number of threads}
  \label{tab:merge-time-800M}
  \begin{tabular}{|c|c|c|c|} \hline
    Number of threads&Time(seconds)\\ \hline
    10&56907 s\\ \hline
    20&30047 s\\ \hline
    30&21387 s\\ \hline
    40&17119 s\\
  \hline\end{tabular}
  \end{table}

  \begin{figure}[t]
    \begin{center}
    \begin{tikzpicture}
    \begin{axis}[
              scale=0.5,
              grid=major, % Display a grid
              grid style={solid,gray!25}, % Set the style
              xmin = 0, xmax = 64,
              ymin = 5, ymax = 60,
              xlabel= Number of threads, % Set the labels
              ylabel=Search latency(ms),
              ylabel shift=-7pt,
              xlabel shift =10pt,
              ytick distance = 10,
              legend columns = 2,
              legend style={at={(0.5, -0.30)},anchor=north},
            ]
            \addplot [red, mark = *, mark size = 0.5pt]table[x=X,y=Y,col sep=space] {MeanSearchLatency_800M.txt}; 
            \addplot [blue, mark = *, mark size = 0.5pt]table[x=X,y=Y,col sep=space] {SearchLatency99_800M.txt}; 
            \legend{Mean Latency, $99^{th}$ percentile latency}
    \end{axis}
    \end{tikzpicture}
    \caption{Trend of mean and 99th percentile latencies for 95\% search
      recall on a 800M SIFT index with different number of threads. Each point is calculated over a search batch of 10000 queries}
    \label{fig:800m-search-latency}
    \end{center}
    \end{figure}

    \begin{figure}[t]
      \begin{center}
      \begin{tikzpicture}
      \begin{axis}[
                scale=0.5,
                grid=major, % Display a grid
                grid style={solid,gray!25}, % Set the style
                xmin = 0, xmax = 64,
                ymin = 150, ymax = 6500,
                xlabel= Number of threads, % Set the labels
                ylabel=Throughput(queries/second),
                ylabel shift=-7pt,
                xlabel shift =10pt,
                ytick distance = 750,
              ]
              \addplot [red, mark = *, mark size = 0.5pt]table[x=X,y=Y,col sep=space] {SearchThroughput_800M.txt}; 
      \end{axis}
      \end{tikzpicture}
      \caption{Trend of search throughput for 95\% search
      recall on a 800M SIFT index with different number of threads}
      \label{fig:800m-search-throughput}
      \end{center}
      \end{figure}

\begin{figure}[t]
  \begin{center}
  \begin{tikzpicture}
  \begin{axis}[
            scale=0.9,
            grid=major, % Display a grid
            grid style={solid,gray!25}, % Set the style
            xmin = 0, xmax = 630000,
            ymin = 0, ymax = 70,
            xlabel= Time elapsed since beginning of experiment (seconds), % Set the labels
            ylabel=Search latency(ms),
            ylabel shift=-7pt,
            xlabel shift =20pt,
            ytick distance = 10
          ]
          \addplot [red, mark = *, mark size = 0.5pt]table[x=X,y=Y,col sep=space] {SteadyState_sift1b_concurr_search_latency.txt}; 
          
  \end{axis}
  \end{tikzpicture}
  \caption{Search latencies for 92\% search
    recall over a week-long experiment of multiple cycles of inserting and deleting 30M points
    concurrently into a 800M SIFT index. Each point is the mean latency over a search batch of 10000 queries}
  \label{fig:steady-800m-search-latency}
  \end{center}
  \end{figure}

  \begin{figure}[ht]
    \begin{center}
    \begin{tikzpicture}
    \begin{axis}[
              scale=0.5,
              grid=major, % Display a grid
              grid style={solid,gray!25}, % Set the style
              xmin = 0, xmax = 40,
              ymin = 550, ymax = 1600,
              xlabel=\#Batches, % Set the labels
              ylabel=Latency($\mu$s),
              ylabel shift=-7pt,                   
              ytick distance = 100,
              legend columns = 3,
              legend style={at={(0.5, -0.30)},anchor=north},
            ]
            \addplot [red, mark = triangle*, mark size = 0.5pt]table[x=X,y=Y1,col sep=space] {SteadyState_sift1b_insertion_latency_percentile.txt}; 
            \addplot [blue, mark = triangle*, mark size = 0.5pt]table[x=X,y=Y2,col sep=space] {SteadyState_sift1b_insertion_latency_percentile.txt}; 
            \addplot [green, mark = triangle*, mark size = 0.5pt]table[x=X,y=Y3,col sep=space] {SteadyState_sift1b_insertion_latency_percentile.txt}; 
            \legend{$10^{th}$, $50^{th}$, $90^{th}$}
    \end{axis}
    \end{tikzpicture}
    \caption{Trend of $10^{th}$, $50^{th}$ and $90^{th}$ percentile user perceived insertion latencies over a week-long experiment of multiple cycles of inserting and
      deleting 30M points concurrently into a 800M SIFT index. Each point is calculated over 30M insertion latencies}
    \label{fig:steady-800m-insert-latency}
    \end{center}
    \end{figure}


==> latency-table.tex <==
\begin{table}[t]
  \centering
  \caption{Mean search latency in microseconds for $95\%$ (top),
    $98\%$ (middle), and $99\%$ (bottom) 5-recall@5.}
  \label{tab:latency}
  \begin{tabular}{|c|c|c|c|} \hline
    Dataset&\algo&\algofresh&HNSW\\ 
    \hline
    SIFT1M&\textbf{93.03} $\mu$s&100.65 &117.48 \\ \hline
    DEEP1M&\textbf{82.03} &87.46 &110.64 \\ \hline
    GIST1M&\textbf{1591.72} &1663.62 &2000.79 \\ \hline
    SIFT100M&\textbf{1646.35} &1714.90 &2414.44 \\ \hline
  \end{tabular}
  %\label{tab:tab2}
  %\end{table*}

  %\begin{table*}
  %\centering
%\caption{Latency for $98\%$ 5-recall@5}
  \begin{tabular}{|c|c|c|c|} \hline
    Dataset&\algo&\algofresh&HNSW\\ 
    \hline
    SIFT1M&\textbf{143.91} &156.18 &193.01 \\ \hline
    DEEP1M&\textbf{132.26} &136.59 &180.701 \\ \hline
    GIST1M&2927.05 &\textbf{2855.56} &3455.59 \\ \hline
    SIFT100M&\textbf{1978.94} &1998.72 &4086.42 \\ \hline
  \end{tabular}
  %\label{tab:tab3}
  %\end{table*}
  
  %\begin{table*}
  %\centering
  %\caption{Latency for $99\%$ 5-recall@5}
  \begin{tabular}{|c|c|c|c|} \hline
    Dataset&\algo&\algofresh&HNSW\\ 
    \hline
    SIFT1M&\textbf{188.90} &207.09 &270.10 \\ \hline
    DEEP1M&\textbf{184.61} &188.94 &246.11 \\ \hline
    GIST1M&4826.52 &\textbf{4535.21} &4670.89 \\ \hline
    SIFT100M&\textbf{2301.15} &2332.57 &5599.45 \\ \hline
  \end{tabular}
\end{table}

==> merge.tex <==
\subsection{The \large{\merger} procedure}

\diskanntwo uses a out-of-memory two-pass streaming merge procedure
that folds newly inserted points in the various instances of
\textbf{RO-\tempindex} into \lti on SSD. During this procedure, points
in the \deletelist are removed from the \lti as well. This procedure
is run in the background and while it runs, the overall system can
still accept insert operations using the active existing
RW-\tempindex. Similarly, delete and search requests can continue to
be served.  Once the merge completes, the system clear outs all the
RO-\tempindex instances which have been merged and also removes those
nodes from the \deletelist whose deletions have been processed in the
\lti.

Like \diskann, the \merge procedure aims to maximize the
\emph{quality} of the resulting index at very low memory footprint. It
does so using the following three-phase algorithm.

\begin{enumerate}
  \item \texttt{DELETE} -- This phase works only on the singleton \lti
    instance and produces an intermediate \lti as output which has removed all the deleted points in \deletelist from the \lti by running Algorithm
    ~\ref{alg:deletion}. To reduce pressure of random reads on
    the disk, we cache $N_{out}(p)\quad \forall p$ in
    \deletelist. This phase loads a block of the \lti file on SSD,
    executes Algorithm~\ref{alg:deletion} for the nodes in the block
    using multiple threads, and writes it back to SSD. There is however a catch:~\Cref{alg:deletion} assumes access to all the full precision vectors which are needed in the invocation to~\Cref{alg:robustprune}. However, the \lti, being a \diskann index stores only the compressed vectors in main memory. So we slightly modify the prune procedure to use the
    \emph{compressed PQ vectors to calculate the approximate distances} needed in~\Cref{alg:robustprune}.
\item \texttt{INSERT} -- For each new point $p$ to be added to \lti
  from \textbf{RO-\tempindex} instances, we use
  Algorithm~\ref{alg:insert} to determine its out-neighbors. To ensure
  all points in \textbf{RO-\tempindex} and \lti are visible to $p$
  during $\greedysearch{\cdot}{v}{\cdot}{\cdot}$, we search for $p$ in
  the \lti instance as well as all the \tempindex instances and take a
  union of all the points visited during the search
  to obtain the visited node list $\mathcal{V}$. The final
  out-neighborhood $N_{out}(p)$ is then computed using the prune
  procedure applied to $\mathcal{V}$ as in~\Cref{alg:insert}. However,
  unlike Algorithm~\ref{alg:insert}, we do not immediately attempt to
  insert $p$ into $N_{out}(p')$ for $p'\in N_{out}(p)$ since this
  could result in an impractical number of random reads and writes to
  the SSDs. Instead, we maintain an in-memory data-structure,
    $\Delta$, to keep track of all such \emph{back edges} to
    add. $\Delta(p)$ is the set of all nodes that need $p$ to add
  themselves to the out-neighbor list of $p$ during the
  \texttt{INSERT} phase.
\item \texttt{PATCH} -- In this phase, we fold the newly inserted
  points and all resulting edges into the \lti. We scan all points $p$ in
  \lti $\cup$ \textbf{RO-\tempindex} $\setminus$ \deletelist (i.e., all the active points in the merged index), and check if any of their new degrees $|\nout{p} \cup \Delta(p)|$ exceeds $R$. If o,  we re-compute the neighborhood by setting $N_{out}(p) =
  \prune{p}{N_{out}(p)\cup \Delta(p)}{\cdot}{\cdot}$ and reflect the
  change on the disk. \emph{Here again, we use the compressed vectors for any distance calculations during the prune procedure. } To perform this operation in an efficient
  manner, we sequentially scan blocks of the \lti file on disk,
  \emph{patch} the new edges and points into the index using the data
  parallel $\prune{\cdot}{\cdot}{\cdot}{\cdot}$ procedure, and writes
  it back to SSD.
\end{enumerate}

%In summary the overall merge process sequentially scans the original


==> plots/merge-scaling-stacked-barchart-pdf.tex <==
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.45\textwidth]{plots/merge_scalability_inv.pdf}
%\includegraphics[width=0.45\textwidth]{plots/merge-scaling.pdf}
\end{center}
\caption{Runtime of \texttt{\merger} with 10, 20, 30 and 40 threads}
\label{fig:merge-scaling}
\end{figure}

==> plots/rebuild-time-table.tex <==
\begin{table}
	\centering
	\caption{Time taken by Vamana versus FreshVamana to reflect same amount of changes to an index - 5\% deletes and inserts}
	\label{tab:vamana-update-time-5percent}
	\begin{tabular}{|c|c|c|} \hline
        Dataset&Vamana(sec)&FreshVamana(sec)\\ \hline
		SIFT1M&32.3s&3.765 s\\ \hline
		DEEP1M&26.9s&3.1935 s\\ \hline
		GIST1M&417.2s&24.3435 s\\ \hline
		SIFT100M&7187.1s&728.723 s\\
		\hline\end{tabular}
\end{table}

\begin{table}
	\centering
	\caption{Time taken by Vamana versus FreshVamana to reflect same amount of changes to an index - 10\% deletes and inserts}
	\label{tab:vamana-update-time-10percent}
	\begin{tabular}{|c|c|c|} \hline
        Dataset&Vamana(sec)&FreshVamana(sec)\\ \hline
		SIFT1M&32.3s&7.0703 s\\ \hline
		DEEP1M&26.9s&6.5057 s\\ \hline
		GIST1M&417.2s&54.6723 s\\ \hline
		SIFT100M&7187.1s&1363.9 s\\
		\hline\end{tabular}
\end{table}

\begin{table}
	\centering
	\caption{Time taken by Vamana versus FreshVamana to reflect same amount of changes to an index - 50\% deletes and inserts}
	\label{tab:vamana-update-time-50percent}
	\begin{tabular}{|c|c|c|} \hline
        Dataset&Vamana(sec)&FreshVamana(sec)\\ \hline
		SIFT1M&32.3s&20.1418 s\\ \hline
		DEEP1M&26.9s&16.0276 s\\ \hline
		GIST1M&417.2s&218.4881 s\\ \hline
        SIFT100M&7187.1s&3914.949 s\\
		\hline\end{tabular}
\end{table}

==> recap.tex <==
\section{Recap of DISKANN}

\begin{algorithm}
\DontPrintSemicolon
\SetAlgoLined
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\KwData{Graph $G(V,E)$ with start node $s$, query point $x_q$, result size $k$, search list size $L$}
\KwResult{Set $\mathcal{L}$ of $k$ nearest neighbors, Set $\mathcal{V}$ of nodes visited and expanded during search}
\BlankLine
 $initialize \ \mathcal{L}\leftarrow \{s\}, \mathcal{V}\leftarrow \emptyset$\;
\BlankLine
\While{$\mathcal{L} \backslash \mathcal{V} \neq \emptyset$}{
$let \ p^* = argmin_{p\in \mathcal{L}\backslash \mathcal{V}}\|x_p - x_q\|$\;
$update \ \mathcal{L}\leftarrow \mathcal{L}\cup N_{out}(p^*)$\;
$update \ \mathcal{V} \leftarrow \mathcal{V} \cup \{p^*\}$\;
\If{$| \mathcal{L}| > L$}{
$update \ \mathcal{L} \ to \ retain \ closest \  L \ points \ to \ x_q$\;
}\;
}
$return \ [closest \ k \ points \ from \ \mathcal{L}, \mathcal{V}]$
\caption{GreedySearch($x_q$, $s$, $k$,$L$)}
\end{algorithm}

\begin{algorithm}
\DontPrintSemicolon
\SetAlgoLined
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\KwData{Graph $G(V,E)$, point $p$, distance threshold $\alpha > 1$, out degree bound $R$, candidate set $\mathcal{V}$}
\KwResult{Set $\mathcal{R}$ containing at most $R$ out neighbors of $p$}
\BlankLine
$initialize \ \mathcal{R} \leftarrow \emptyset$\;
\While{$\mathcal{V} \neq \emptyset$}{
$let \ p^* = argmin_{p'\in \mathcal{V}}\|x_p - x_{p'}\|$\;
$\mathcal{R} \leftarrow \mathcal{R} \cup \{p'\}$\;
\eIf{$|\mathcal{R}| > R$}{
$break$\;
}{
\ForEach{$p' \in \mathcal{V}$}{
\If{($\alpha * \|x_p - x_p*\| < \|x_p - x_p'\|$)}{
$remove \ p' from \ \mathcal{V}$\;
}
}
}
}
$return \ \mathcal{R}$
\caption{PruneNeighbors($p$, $\alpha$, $R$, $\mathcal{V}$)}
\end{algorithm}

